Relation Prediction as an Auxiliary Training Objective for Improving Multi-Relational Graph Representations

Learning good representations on multi-relational graphs is essential to knowledge base completion (KBC). In this paper, we propose a new self-supervised training objective for multi-relational graph representation learning, via simply incorporating relation prediction into the commonly used 1vsAll objective. The new training objective contains not only terms for predicting the subject and object of a given triple, but also a term for predicting the relation type. We analyse how this new objective impacts multi-relational learning in KBC: experiments on a variety of datasets and models show that relation prediction can significantly improve entity ranking, the most widely used evaluation task for KBC, yielding a 6.1% increase in MRR and 9.9% increase in Hits@1 on FB15k-237 as well as a 3.1% increase in MRR and 3.4% in Hits@1 on Aristo-v4. Moreover, we observe that the proposed objective is especially effective on highly multi-relational datasets, i.e. datasets with a large number of predicates, and generates better representations when larger embedding sizes are used.

==> tables/1.tex <==
\begin{table}[htb]
\centering

\begin{tabular}{llll}
\toprule
Model &         MRR &      Hits@1 &       Hits@3 \\
\midrule
\rowcolor{lightgray} RESCAL   &  0.36 (0\%)   &  0.27 (0\%)   &  0.39 (0\%)   \\
                     CP       &  0.36 (+3\%)  &  0.27 (+4\%)  &  0.39 (0\%)   \\
\rowcolor{SkyBlue} ComplEx  &  0.38 (+3\%)  &  0.29 (+7\%)  &  0.42 (+5\%)  \\
                     TuckER   &  0.33 (+3\%)  &  0.24 (0\%)  &  0.36 (+3\%)  \\
\bottomrule
\end{tabular}
%\end{adjustbox}

\caption{Perturbing Relations Across Models on FB15k-237. Percentages indicate the relative change brought by the MLM-styled objective over the traditional one.}
\label{tab:across_model}
\end{table}



==> tables/13_performance_both.tex <==
\begin{table*}[t]
    \centering
% \begin{tabular}{rcccccc}
% \toprule
% \multirow{2}{*}{\bf Metric} & \multicolumn{3}{c}{\bf Relation perturbation} & \multicolumn{3}{c}{\bf Weighted Relation Perturbation} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%  &             {\bf Aristo-v4} &     {\bf FB15K-237} &        {\bf WN18RR} &                      {\bf Aristo-v4} &     {\bf FB15K-237} &        {\bf WN18RR} \\
% %Metric  &                       &               &               &                                &               &               \\
% \midrule
% Hits@1  &          0.24 (+2.4\%) &  0.29 (+6.6\%) &  0.43 (-2.4\%) &                   0.24 (+3.4\%) &   0.3 (+9.9\%) &  0.44 (+0.4\%) \\
% Hits@10 &          0.45 (+2.2\%) &  0.57 (+2.0\%) &  0.56 (-3.4\%) &                   0.45 (+2.1\%) &  0.57 (+2.1\%) &  0.58 (-0.3\%) \\
% Hits@3  &          0.33 (+2.8\%) &  0.42 (+4.5\%) &  0.49 (-2.6\%) &                   0.34 (+3.8\%) &  0.43 (+6.1\%) &   \ 0.5 (+0.8\%) \\
% MRR     &          0.31 (+2.3\%) &  0.38 (+4.5\%) &  0.47 (-2.8\%) &                   0.31 (+3.1\%) &  0.39 (+6.1\%) &  0.49 (+0.3\%) \\
% \bottomrule
% \end{tabular}
\resizebox{\textwidth}{!}{%
\begin{tabular}{rllllll}
\toprule
% Type & \multicolumn{3}{l}{Relation Perturbation} & \multicolumn{3}{l}{Weighted Relation Perturbation} \\
% {} &                WN18RR &     FB15K-237 &     Aristo-v4 &                         WN18RR &     FB15K-237 &     Aristo-v4 \\
\multirow{2}{*}{\bf Metric} & \multicolumn{3}{c}{\bf Relation perturbation} & \multicolumn{3}{c}{\bf Weighted Relation Perturbation} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
&             {\bf WN18RR}  &     {\bf FB15k-237} &   \bf {Aristo-v4} &  {\bf WN18RR} & {\bf FB15k-237} & {\bf Aristo-v4}\\
\midrule
MRR     &          0.47 (-2.8\%) &  0.38 (+4.5\%) &  0.31 (+2.3\%) &                   0.49 (+0.3\%) &  0.39 (+6.1\%) &  0.31 (+3.1\%) \\
Hits@1  &          0.43 (-2.4\%) &  0.29 (+6.6\%) &  0.24 (+2.4\%) &                   0.44 (+0.4\%) &   0.3 (+9.9\%) &  0.24 (+3.4\%) \\
Hits@3  &          0.49 (-2.6\%) &  0.42 (+4.5\%) &  0.33 (+2.8\%) &                    0.5 (+0.8\%) &  0.43 (+6.1\%) &  0.34 (+3.8\%) \\
Hits@10 &          0.56 (-3.4\%) &  0.57 (+2.0\%) &  0.45 (+2.2\%) &                   0.58 (-0.3\%) &  0.57 (+2.1\%) &  0.45 (+2.1\%) \\
\bottomrule
\end{tabular}
}
    \caption{ComplEx with (Weighted) Relation Perturbation across datasets, absolute values rounded to 2 digits. Percentages indicate the relative change brought by (weighted) relation perturbation over no relation perturbation. }
    \label{tab:performance_both}
\end{table*}

==> tables/2.tex <==
\begin{table}[htb]
    \centering
%\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{lllll}
\toprule
Rank &    MRR & Hits@1 & Hits@3 & Hits@10 \\
\midrule
500  &  \cellcolor[HTML]{3CB371} +1.2\% &  \cellcolor[HTML]{00FF7F} +3.2\% & \cellcolor[HTML]{006400} -0.6\% & \cellcolor[HTML]{006400} -0.5\% \\
1000 &  \cellcolor[HTML]{00FA9A} +2.2\% &  \cellcolor[HTML]{3CB371} +1.9\% & \cellcolor[HTML]{00FF7F} +3.1\% & \cellcolor[HTML]{3CB371} +1.8\% \\
1500 &  \cellcolor[HTML]{00FA9A} +2.3\% &  \cellcolor[HTML]{00FA9A} +2.4\% & \cellcolor[HTML]{00FA9A} +2.8\% & \cellcolor[HTML]{00FA9A} +2.2\% \\
2000 &  \cellcolor[HTML]{2E8B57} +0.7\% &  \cellcolor[HTML]{3CB371} +1.1\% & \cellcolor[HTML]{2E8B57} +0.4\% & \cellcolor[HTML]{2E8B57} +0.8\% \\
\bottomrule
\end{tabular}
%\end{adjustbox}
    \caption{Relative change of MRR, Hits@1, Hits@3 and Hits@10 on Aristo-v4 dataset. ComplEx with different ranks were trained and the hyper-parameters were chosen based on the validation MRR. Note that the numbers are in percentage. Brighter colours indicate a larger improvement introduced by the relation prediction objective.}
    \label{tab:aristo-v4}
\end{table}

==> tables/4.tex <==
\begin{table}[t]
    \centering
\begin{tabular}{lllll}
\toprule
{} &   MRR & hits@1 & hits@3 & hits@10 \\
Model   &       &        &        &         \\
\midrule
TransE  &  0.23 &      - &      - &    0.52 \\
\rowcolor{SkyBlue} RNN     &  0.42 &   0.38 &   0.43 &    0.49 \\
ConvE   &  0.43 &   0.40 &   0.44 &    0.52 \\
ComplEx &  0.49 &   0.44 &   0.50 &    0.58 \\
\bottomrule
\end{tabular}
    \caption{RNN-KBC Compared with Classic Knowledge Base Completion Models on WN18RR. 
    The result of TransE and ConvE are taken from literature \cite{dettmers2018convolutional, Teach2020YouCT}. For RNN and ComplEx, 
    we used N3 regularizer and embedding sizes of 1000. 
    Hyper-parameters are chosen based on the best validation MRR.}
    \label{tab:rnn_kbc}
\end{table}

==> tables/6_performance_dataset_vanila.tex <==

%MERGE TABLE 2 AND TABLE 3
\begin{table*}[htb]
    \centering
\begin{tabular}{lllll}
%\toprule
Dataset &           MRR &        Hits@1 &        Hits@3 &       Hits@10 \\
% Dataset   &               &               &               &               \\
\midrule
WN18RR    &  $0.47 (-2.8\%)$ &  $0.43 (-2.4\%)$ &  $0.49 (-2.6\%)$ &  $0.56 (-3.4\%)$ \\
FB15k-237 &  $0.38 (+4.5\%)$ &  $0.29 (+6.6\%)$ &  $0.42 (+4.5\%)$ &  $0.57 (+2.0\%)$ \\
Aristo-v4 &  $0.31 (+2.3\%)$ &  $0.24 (+2.4\%)$ &  $0.33 (+2.8\%)$ &  $0.45 (+2.2\%)$ \\
%\bottomrule
\end{tabular}
    \caption{ComplEx with Relation Perturbation across datasets.  Absolute values rounded to 2 digits. Percentage indicate weighted relative change brought by relation perturbation over no relation perturbation. %REPORT ABSOLUTE VALUES ONLY. INCLUDING THE BASELINE MODELS
    }
    \label{tab:performance_dataset_vanila}
\end{table*}

==> tables/7_best_dataset_vanila.tex <==
\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{llrrrrr}
\toprule
          &       &  Rank &  Learning rate &  Batch size &  Regularisation &   Dev MRR \\
Dataset & Relation Perturbation &       &                &             &                 &           \\
\midrule
WN18RR & False &  1000 &           0.10 &         100 &            0.10 &  0.488083 \\
          & True  &  1000 &           0.10 &        1000 &            0.05 &  0.477088 \\
FB15k-237 & False &  1000 &           0.10 &         100 &            0.05 &  0.372305 \\
          & True  &  1000 &           0.10 &        1000 &            0.05 &  0.387133 \\
Aristo-v4 & False &  1500 &           0.01 &         500 &            0.01 &  0.307076 \\
          & True  &  1500 &           0.10 &         100 &            0.05 &  0.313236 \\
\bottomrule
\end{tabular}
\end{adjustbox}
    \caption{Best hyper-parameter configurations and the corresponding validation MRR for ComplEx across datasets with Relation Perturbation}
    \label{tab:best_dataset_vanila}
\end{table*}
